Comparing Apples to Apples: Generating Aspect-Aware Comparative Sentences from User Reviews

It is time-consuming to find the best product among many similar alternatives. Comparative sentences can help to contrast one item from others in a way that highlights important features of an item that stand out. Given reviews of one or multiple items and relevant item features, we generate comparative review sentences to aid users to find the best fit. Specifically, our model consists of three successive components in a transformer: (i) an item encoding module to encode an item for comparison, (ii) a comparison generation module that generates comparative sentences in an autoregressive manner, (iii) a novel decoding method for user personalization. We show that our pipeline generates fluent and diverse comparative sentences. We run experiments on the relevance and fidelity of our generated sentences in a human evaluation study and find that our algorithm creates comparative review sentences that are relevant and truthful.

==> old.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{lc}
        \toprule
        \toprule
         \textbf{Review Examples:}\\
         \midrule
         1. I loved this piano. The Yamaha has a great
          sound for an affordable price. \\
        \midrule    
        2. This cable is great, its length was good and
         very sturdy.\\
        \midrule  
        \textbf{Comparative Review Examples:} \\
        \midrule
         1. Probably the best option to go with. The 
         Yamaha sounds way better than the Roland FP.\\
         \midrule
         2. The amazon cable is much sturdier than 
         the hp cable. \\
         \bottomrule
         \bottomrule
    \end{tabular}
    \caption{In contrast to regular reviews, our work aims to generate comparative review sentences that might be more helpful for purchase decision making from a gamut of product options.}
  \label{tab:my_label}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l}
    \toprule
    \toprule
    \textbf{Contrastive Sentences Classified by BERT}\\
    \midrule
         Minimal pause between songs -- less than that 
         on other devices -- [...]\\
         \midrule
         It is even better than my trusty Shure SM58 \\
         \midrule
         It sounds better than the more expensive 
         Ortofon [...]\\
         \midrule
         In terms of functionality [...] PostgresSQL is 
         much better than MySQL.\\
         \midrule
         That's much better than the Youtube popular 
         blue yeti [...]\\
         \midrule
         So, moldy bread is safer than moldy pizza.\\
         \midrule
        Much better than m65 pro, even though it is 
        more expensive.\\
         \bottomrule
         \bottomrule
    \end{tabular}
    \caption{Instances classified as comparative by our non domain-specific fine-tuned BERT classifier. Very confident predictions ($>90\%$) are used in the further pipeline of our project.}
    \label{tab:my_label}
    \end{table*}
